Protecting GNSS-based Services using Time Offset Validation

Global navigation satellite systems (GNSS) provide pervasive accurate positioning and timing services for a large gamut of applications, from Time based One-Time Passwords (TOPT), to power grid and cellular systems. However, there can be security concerns for the applications due to the vulnerability of GNSS. It is important to observe that GNSS receivers are components of platforms, in principle having rich connectivity to different network infrastructures. Of particular interest is the access to a variety of timing sources, as those can be used to validate GNSS-provided location and time. Therefore, we consider off-the-shelf platforms and how to detect if the GNSS receiver is attacked or not, by cross-checking the GNSS time and time from other available sources. First, we survey different technologies to analyze their availability, accuracy, and trustworthiness for time synchronization. Then, we propose a validation approach for absolute and relative time. Moreover, we design a framework and experimental setup for the evaluation of the results. Attacks can be detected based on WiFi supplied time when the adversary shifts the GNSS provided time, more than 23.942us; with Network Time Protocol (NTP) supplied time when the adversary-induced shift is more than 2.046ms. Consequently, the proposal significantly limits the capability of an adversary to manipulate the victim GNSS receiver.

==> accuracy.tex <==
\subsubsection{Accuracy Analysis}
In order to verify the GPS time, we need to obtain the accuracy, $\epsilon_{ext}$, of each technology, as shown in Eqs. \ref{eq:ext_absolute} and \ref{eq:ext_relative}.
%Each time provider has to be classified in respect of its accuracy to extract a minimum $T_{window}$ and a threshold $\epsilon_{ext}$ based upon its accuracy.  
The accuracy of each technology is obtained by comparing its time information with a GNSS disciplined oscillator. 

For the case of NTP, the accuracy is calculated based upon the offset between the GNSS-provided time and the NTP servers provided time. The left plot of Fig. \ref{fig:ntp_accuracy} shows the offset of three different NTP servers located in the same country as the host, for a period of 22 hours. We use 99\% quantile of each server offset as its accuracy, as shown in right plot of Fig. \ref{fig:ntp_accuracy}, to represent our parameter $\epsilon_{ext}$. And the highest value among the three $\epsilon_{ext}$ is chosen to set the threshold for the NTP time. Therefore, we have:
\begin{equation}
\epsilon_{NTP} = 2.046 \text{ ms}
\label{eq:ntp_accuracy}
\end{equation}
\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{figures/ntp_accuracy.eps}
	\caption{Statistics of three NTP servers}
	\label{fig:ntp_accuracy}
\end{figure}
%\begin{multicols}{2}

A similar approach is used to profile WiFi beacons. In default, APs transmit beacons at a 100 Time Unit (TU, corresponds to 1024 microseconds) \cite{geier2002802}. The accuracy of the WiFi beacons is calculated over three different observation windows, set by $T_{window}=\{1000,\ 3000\ ,5000\}$~TU. And, the difference between the timestamp of the received beacon at the end of the observation window and the timestamp of the beacon at the beginning of the window is $T^{B_{end}}_{AP}-T^{B_{begin}}_{AP}$. Further, the error between this difference and the GNSS disciplined clock measured $T_{window}$ is used to determine the accuracy for WiFi beacons, as presented in Fig. \ref{fig:ap_accuracy}. The left plot is the offset of recorded APs data during each $T_{window}$ comparing with the GNSS disciplined clock measured $T_{window}$, and the right plot gives their 99\% quantile statistics.
\begin{figure*}[!t]
	\centering
	\includegraphics[width=0.9\textwidth,height=2.8in]{figures/ap_accuracy.eps}
	\caption{Statistics of three access points (AP)}
	\label{fig:ap_accuracy}
\end{figure*}
Same as NTP, we choose the highest value of the quantiles among the three APs for each $T_{window}$ as its accuracy:
\begin{equation}
\epsilon_{WiFi} = \Big\{ \begin{array}{cc}
46.064 \text{ $\mu$s}& \qquad T_{window}=1024 \text{ ms} \\
35.021 \text{ $\mu$s}& \qquad T_{window}=3072 \text{ ms} \\
23.942 \text{ $\mu$s}& \qquad T_{window}=5120 \text{ ms}
\end{array}
\label{eq:wifi_accuracy} 
\end{equation}

%$$ Acc_{AP} = (T_{RX}^{B_2} - T_{RX}^{B_1}) - T_{Window} $$

%The $\epsilon_{extk}$ is calculated as the 90\% quantile of each accuracy measurement. The $\epsilon_{ext}$ is chosen conservatively as the highest quantile among the different APs for each $T_{window}$. Figure \ref{fig:ap_accuracy} plots the accuracy of three independent APs over three different observation windows of 1,3,5 seconds.


%\end{multicols}

==> discussion.tex <==
\section{Further Discussion}
\label{sec:discussion}
The proposed concept is to protect a GNSS receiver with other technologies, in which sense the level of trustworthiness of these technology candidates affects the security performance of the proposal. In specific, the lack of authentication in the WiFi beacons represents a substantial limitation of the system. Broadcasting bogus WiFi beacons is not hard, and it would be possible for an attacker to emulate a set of access points to be able to \textcolor{red}{mask the alteration caused to the GNSS timing}. As aforementioned, the implementation of NTPSec allows for securing time transfer from designated NTP servers, defining a higher level of security compared to plain NTP. In addition to the security features of these technologies, the algorithm can be modified to rank the verification sources, based not only on their precision but also on the perceived level of trust, as specified in Eq \ref{eq:gt} in Section \ref{sec:multiple_ext_ts}.

%The addition of authenticated payloads to WiFi beacons would make the system more robust against attackers disseminating bogus beacons. In this context, we suggest the definition of a timing dedicated beacon, that in the optional part of the payload contains an authenticated high precision time information. Such a service would need to be integrated in an infrastructure providing certified identities for each AP in the system which can be made available through the service provider or via subscription. The definition of such a dedicated packet, would allow the WiFi base stations not only to authenticate their relative timing information, but also to broadcast an high precision absolute time reference with message authentication dependent on the implementation of a synchronization method between the different APs. In such a configuration, it would be possible to cross validate the information disseminated by the different APs to detect faults or malicious transmitters as each AP would also be able to verify the timing information distributed by the stations in its surroundings. In the same way, other users of the system, can leverage this to cooperatively identify a subset of stations that can be trusted. Binding the identity of the transmitting station and timing information that it distributes allows for accountability of the disseminated time and raises the complexity for a potential attacker.

==> setup.tex <==
\subsection{Experimental Setup}
%Integrating a gamut of different time sources requires system wide clock access to correlate independent channels. One of the main challenges in this approach, is to make the individual times to be comparable. Wireless opportunistic beacons, internal clocks, remote timing servers are all valid options to acquire high precision time signals, but the way this information can be accessed by the system is critically different. A combination of synchronous and asynchronous processes creates significant challenges in combining the information obtained by the time sources, with a need to define a common time reference. Opportunistic radio beacons advertise their information without the client to be able to control the emission time. WiFi beacons are transmitted without any form of synchronization among different Access Points (AP) and at user configurable rates. These characteristic make the reception of beacons completely asynchronous in respect of the receiving system. On the other hand, the emission rate of the GNSS timing information is dependent on the solution rate of the GNSS receiver. The predictability of the message arrival time makes this information available synchronously and at the receiver rate. Other services, like NTP, are purely on-demand and they depend on the request rate of the client. NTP has limitations on the maximum rate of requests. Most NTP providers limit the minimum polling rate to 6 seconds.
%
%Combining all these approaches to produce comparable time scales is not an easy task. The approach used in this work leverages the consistency that can be provided by a single time collection endpoint. While each service could produce data at its own rate, working asynchronously from the rest of the modules, one central endpoint collects the information produced by each service and aligns the timescales to make the comparable. The reference used to align the timescales is provided by the system clock. When each service produces a new message, the arrival time of the message is recorded and appended to the data before it is sent to the central service.
%In this work, the GNSS and NTP services are tightly interconnected, using the arrival of the GNSS time to generate an event triggering the NTP request. This approach is used to minimize the effort in compensating for delays between the two services. Due to the limitations imposed by the minimum polling time of NTP servers, one NTP request is generated every tenth GPS message. 

In this work, we leverage two external time services, NTP and WiFi beacons, to verify the GPS time, as presented in Fig. \ref{fig:setup}. The  ublox EVK-6T evaluation kit \cite{ublox2012} offers two interfaces for data transmission: a USB2 port provides a real-time PVT solution that the manipulated GPS time is synthesized based on; a RS232 serial port provides a GPS time pulse for the host synchronization. The serial port provides a high accuracy pulse per second (PPS) via the Data Carrier Detect (DCD) pin, which is used as a reference to check the performance of the evaluation results.

Besides the GPS receiver, other configuration of the setup is as following:
\begin{itemize}
	\item Host machine: Intel I7 CPU running a Linux system whose kernel supports high precision timing
	\item Host WiFi card: Intel Corporation Wireless-AC 9260
	\item WiFi beacons: from surrounding access points of the office building
	\item NTP servers: three servers in Sweden
	\item GPS PVT rate: \SI{1}{Hz}
	\item Observation window candidates for APs: $T_{window}=\{1024,\ 3072\ ,5120\}$~ms
\end{itemize}

%Each component is designed as an independent module to allow reconfiguration. We use a commercially available, off the shelf, GNSS receiver specifically designed for timing services. The UBlox EVK-6T evaluation kit supports multiconstellation receiver configurations and allows for sub microsecond timing precision. Although we mainly use the GPS part of the receiver in this work, the time information provided by different constellations can be used to increase the robustness of the implementation. This approach is left for future work. The evaluation kit offers two communication interfaces, one USB2.0 used to interface the replay detection system with the GNSS receiver and a RS232 serial port used for the host synchronization. The serial port provides a high accuracy pulse per second (PPS) via the Data Carrier Detect (DCD) pin. This feature is used for validation measurements as it provides a stable synchronization pulse. This is important because, during the evaluation phase, the profiling clock needs to be more accurate than the clock under test.

%For the host computer, we use Linux operating system with kernel support for high precision timing. The host machine uses an "Intel i7 cpu with 16gb of RAM". To provide wireless connectivity, we use an Intel WiFi card for beacon monitoring and the host has internet connectivity. The verification system comprises three main blocks. The WiFi monitoring application scans for beacons and timestamps the arrival time of each beacon. The application selects a pool of beacons to observe among those available in the area by choosing the closest ones to the user considering the RSSI value. Checking for good availability before starting the monitoring phase is important to make sure the system obtains a valid and stable set of beacons before using them to validate the GNSS timing information. In addition to this, using a subset of the available beacons reduces the performance bottleneck that might happen in crowded WiFi environments. The content of sampled beacons is streamed to the controller application over a low latency socket. Upon detection of a GPS time update, the GNSS monitoring application streams a packet containing the system reception time and the GPS synchronized time to the controller and triggers a request to the NTP time server. The controller independently receives these events and aligns the timescales. This architecture allows to deploy the system in a single host or a network of synchronized independent machines, allowing for scalable, easy to update deployments. Figure \ref{fig:system} gives an architecture overview of the experimental setup.
%\begin{figure}[!th]
%	\label{fig:system}
%	\centering
%	\includegraphics[width=\linewidth]{figures/system.pdf}
%	\caption{Architecture of the system used to profile the different time sources, analyze the results and detect the spoofer. Modularity of the design allows for centralized or synchronized distributed deployments}
%\end{figure}


